Fast and accurate solvers for simulating Janus particle suspensions in Stokes flow

We present a novel computational framework for simulating suspensions of rigid spherical Janus particles in Stokes flow. We show that long-range Janus particle interactions for a wide array of applications may be resolved using fast, spectrally accurate boundary integral methods tailored to polydisperse suspensions of spherical particles. These are incorporated into our rigid body Stokes platform. Our approach features the use of spherical harmonic expansions for spectrally accurate integral operator evaluation, complementarity-based collision resolution, and optimal O(n) scaling with the number of particles when accelerated via fast summation techniques. We demonstrate the flexibility of our platform through three key examples of Janus particle systems prominent in biomedical applications: amphiphilic, bipolar electric and phoretic particles. We formulate Janus particle interactions in boundary integral form and showcase characteristic self-assembly and complex collective behavior for each particle type.

==> results.tex <==
\label{sec:Results}
In this section we perform a numerical validation of our evaluation algorithm for the Janus particle potentials. 
For these experiments, as in the aforementioned studies, we used a serial Matlab implementation of the simulation algorithm. The FMM libraries \cite{gimbutas2012stfmmlib3,greengard2012fmmlib3d} are originally implemented in C++ and are called through a mex wrapper. Our simulations were then run on the Flux cluster at the University of Michigan. 


\subsection{Validation}
We construct a simple boundary value problem to test the accuracy of our near evaluation routine.
\begin{figure}[H]
\centering
\subfloat[Subfigure 1 list of figures text][]{
\includegraphics[width=0.5\textwidth]{images/BIE_ERROR_PLOT_SPHERES.png}
\label{fig:spheretest}}
\subfloat[Subfigure 3 list of figures text][]{
\includegraphics[width=0.5\textwidth]{images/BIE_ERROR_PLOT.png}
\label{fig:sphereerror}}
\qquad
\label{fig:BIE_validation}
\caption{Distribution of error for $p=8, k=2$ (a) and error ranges (b)}
\end{figure}

 We take three spheres located at (-1.5, 1, 0), (-3, 0, 0), (-1, 0, 2) and with radius $r_i = 0.5, 1 , 0.7$ respectively.  We place a positive point charge of unit strength at interior position $x_i$ for $i=1,2,3.$ $x_i$ is located a distance of $\frac{r_i}{10}$ from the center of sphere $i$. The potential at an arbitrary point can be directly computed as 
 \begin{equation}
 \phi(x) = \sum_{i=1}^3 G_\lambda(x_i,x)
 \end{equation}
 
 
  Alternatively, the above formula can be used to compute the values of the potential on the surface of the sphere and a Dirichlet boundary problem can be solved to compute the potential at points in the exterior as per equation \ref{eq:DirichletBd}. This allows us a method of computing the accuracy of the evaluation routine we have developed. In this test, all target points are near enough that the spherical harmonic subroutine is used. We evaluate the potential on the surface of target spheres concentric to the source spheres, with target sphere $i$ having radius $r_i + 10^{-k}$ for $k=1,2...$. While the layer potentials become more and more singular,  the error decays spectrally as p is increased and does not decay as the target radius decreases. \ref{fig:spheretest} plots the error at points on the target spheres for $p=8, k=2$, \ref{fig:sphereerror} shows the range of error for different values of $p,k$.

\begin{comment}
\subsection{Numerical Properties}   
The linear systems obtained from BIE  discretization have, by design, a moderately sized and bounded condition number. We randomly perturb a regular cubic lattice with a distance of 4 radii between particle centers. We record below the condition number for systems of 1,8,27, and 64 particles. Figure \ref{fig:cond_number_test} Shows how the condition number grows with the number of particles for different values of lambda. We observe that larger values of lambda lead to smaller condition numbers.


Next we investigate how the number of GMRES iterations depend on the minimum distance between particles. We place four particles at varying minimum  distances from each other and compute the average over ten timesteps, plotting the result in \ref{tab:mindist}. The minimum distance increases from 0.2 to 0.5 1, and 8.  We observe that the number of GMRES iterations remains low for the bipolar particles. As the distance increases, the condition number decreases.
\end{comment}
\begin{comment}
\begin{table}[H]
    \centering
    \begin{tabular}{|c|c|c|c|c|}
\hline
Number of particles &  GMRES (A) & GMRES (B) & $\kappa_A$ & $\kappa_B$ \\
\hline
1 & 2 & 3 & 1.87 & 1.58 \\
\hline
8 & 7 & 6.00 & 3.43 & 1.76 \\
\hline
27 & 9 & 6.19 & 5.63 & 5.47  \\
\hline
64 & 10 & 6 & 8.00 & 19.71 \\
\hline 
\end{tabular}
    \caption{Number of GMRES iterations and condition number for Amphiphilic (A) and Bipolar (B) systems}
    \label{tab:condition}
\end{table}

\begin{table}[H]
    \centering
    \begin{tabular}{|c|c|c|}
\hline
Minimum Distance & GMRES(A) & GMRES(B) \\
\hline
8 & 5.00 & 5.00 \\
\hline
1 & 8.00 & 7.07 \\
\hline
0.5 & 9.96 & 7.58\\
\hline
0.2 & 11.11 & 7.58\\
\hline
\end{tabular}
    \caption{Number of GMRES iterations vs minimum distance for 4 particle configurations of Amphiphilic (A) and Bipolar (B) systems }
    \label{tab:mindist}
\end{table}
\end{comment}




